Bottleneck Conditional Density Estimation

We introduce a new framework for training deep generative models for high-dimensional conditional density estimation. The Bottleneck Conditional Density Estimator (BCDE) is a variant of the conditional variational autoencoder (CVAE) that employs layer(s) of stochastic variables as the bottleneck between the input $x$ and target $y$, where both are high-dimensional. Crucially, we propose a new hybrid training method that blends the conditional generative model with a joint generative model. Hybrid blending is the key to effective training of the BCDE, which avoids overfitting and provides a novel mechanism for leveraging unlabeled data. We show that our hybrid training procedure enables models to achieve competitive results in the MNIST quadrant prediction task in the fully-supervised setting, and sets new benchmarks in the semi-supervised regime for MNIST, SVHN, and CelebA.

==> figures/2z_models.tex <==
\begin{figure*}[!t]
\centering
\subfigure[]{
\begin{tikzpicture}
\node[circ] (z1) {$z_1$};
\node[circ, yshift=-2cm] (x) {$x$};
\path
%% generative model
(z1) edge [connect, pink] (x)
(x) edge [rdotconnect, red] (z1)
;
\end{tikzpicture}
\label{fig:vaex}
}
\subfigure[]{
\begin{tikzpicture}
\node[circ] (z1) {$z_1$};
\node[circ, xshift=+2cm] (z2) {$z_2$};
\node[circ, xshift=+2cm, yshift=-2cm] (y) {$y$};
\path
%% generative model
(z1) edge [connect, green!50!black] (z2)
(z2) edge [connect, blue] (y)
(y) edge [ldotconnect] (z1)
(y) edge [rdotconnect, brown] (z2)
;
\end{tikzpicture}
\label{fig:vaey}
}
\subfigure[]{
\begin{tikzpicture}
\node[circ] (z1) {$z_1$};
\node[circ, xshift=+2cm] (z2) {$z_2$};
\node[circ, yshift=-2cm] (x) {$x$};
\node[circ, xshift=+2cm, yshift=-2cm] (y) {$y$};
\path
%% generative model
(z1) edge [connect, pink] (x)
(z1) edge [connect, green!50!black] (z2)
(z2) edge [connect, blue] (y)
(x) edge [rdotconnect, gray] (z1)
(y) edge [dotconnect, gray, bend left=15] (z1)
(y) edge [rdotconnect, brown] (z2)
;
\end{tikzpicture}
\label{fig:vaexy}
}
\subfigure[]{
\begin{tikzpicture}
\node[circ] (z1) {$z_1$};
\node[circ, xshift=+2cm] (z2) {$z_2$};
\node[circ, yshift=-2cm] (x) {$x$};
\node[circ, xshift=+2cm, yshift=-2cm] (y) {$y$};
\path
%% generative model
(x) edge [connect, red] (z1)
(z1) edge [connect, green!50!black] (z2)
(z2) edge [connect, blue] (y)
(x) edge [rdotconnect, gray] (z1)
(y) edge [dotconnect, gray, bend left=15] (z1)
(y) edge [rdotconnect, brown] (z2)
;
\end{tikzpicture}
\label{fig:cvae}
}
\caption{The joint and conditional components of a 1-layer BCDE. Dotted lines represent recognition models. Colors indicate the parameters that are strictly tied within the joint model and softly tied between the joint and conditional models.}\label{fig:models}
\end{figure*}


==> figures/bde.tex <==
\begin{figure}[!t]
\centering
\begin{tikzpicture}
\node[circ] (zp) {$z$};
\node[circ, xshift=-1.5cm, yshift=-1.5cm] (xp) {$x$};
\node[circ, xshift=+1.5cm, yshift=-1.5cm] (yp) {$y$};
\node[draw, rectangle, rounded corners, minimum width=4.5cm, minimum height=3.5cm, yshift=-0.5cm]    {};
\node[none, yshift=+0.8cm] {BJDE};

\node[circ, xshift=+8cm] (z) {$z$};
\node[circ, xshift=+6.5cm, yshift=-1.5cm] (x) {$x$};
\node[circ, xshift=+9.5cm, yshift=-1.5cm] (y) {$y$};
\node[rrec, xshift=+8cm, yshift=-0.5cm]    {};
\node[none, xshift=+8cm, yshift=+0.8cm] {BCDE};

\node[none, xshift=+4cm] {Regularization};
\node[circ, xshift=+2cm, yshift=-0.3cm, draw=none] (s) {};
\node[circ, xshift=+6cm, yshift=-0.3cm, draw=none] (e) {};
\node[none, xshift=0cm, yshift=-2.3cm] (j) {};
\node[none, xshift=8cm, yshift=-2.3cm] (c) {};
\node[none, xshift=0cm, yshift=-4cm, text width=3cm, align=center] (u) {Unpaired Data\\$\set{x_i} \cup \set{y_i}$};
\node[none, xshift=4cm, yshift=-4cm, text width=3cm, align=center] (p) {Paired Data\\$\set{x_i, y_i}$};

\path
%% generative model
(zp) edge [connect] (xp)
(zp) edge [connect] (yp)
(xp) edge [rdotconnect, bend right=45] (zp)
(yp) edge [ldotconnect, bend left=45] (zp)
(x) edge [connect] (z)
(z) edge [connect] (y)
(x) edge [rdotconnect, bend right=45] (z)
(y) edge [ldotconnect, bend left=45] (z)
(s) edge [bothconnect] (e)
(u) edge [connect] (j)
(p) edge [connect] (j)
(p) edge [connect] (c)
;
\end{tikzpicture}  
\caption{The hybrid training procedure that regularizes the BCDE toward the BJDE. This regularization enables the BCDE to indirectly leverage unpaired $x$ and $y$ for conditional density estimation.}
\label{fig:bde}
\end{figure}
